Payoff-based learning with matrix multiplicative weights in quantum games

In this paper, we study the problem of learning in quantum games - and other classes of semidefinite games - with scalar, payoff-based feedback. For concreteness, we focus on the widely used matrix multiplicative weights (MMW) algorithm and, instead of requiring players to have full knowledge of the game (and/or each other's chosen states), we introduce a suite of minimal-information matrix multiplicative weights (3MW) methods tailored to different information frameworks. The main difficulty to attaining convergence in this setting is that, in contrast to classical finite games, quantum games have an infinite continuum of pure states (the quantum equivalent of pure strategies), so standard importance-weighting techniques for estimating payoff vectors cannot be employed. Instead, we borrow ideas from bandit convex optimization and we design a zeroth-order gradient sampler adapted to the semidefinite geometry of the problem at hand. As a first result, we show that the 3MW method with deterministic payoff feedback retains the $\mathcal{O}(1/\sqrt{T})$ convergence rate of the vanilla, full information MMW algorithm in quantum min-max games, even though the players only observe a single scalar. Subsequently, we relax the algorithm's information requirements even further and we provide a 3MW method that only requires players to observe a random realization of their payoff observable, and converges to equilibrium at an $\mathcal{O}(T^{-1/4})$ rate. Finally, going beyond zero-sum games, we show that a regularized variant of the proposed 3MW method guarantees local convergence with high probability to all equilibria that satisfy a certain first-order stability condition.

==> Body/B-MMW_05_15.tex <==
%----------------------------------------------------------------------
%%% B-MMW
%----------------------------------------------------------------------
% !TEX root = ../Main.tex

In an online learning framework, it is more realistic to consider that players observe only the impact of the \emph{realized} outcome of their actions, \ie
each player $\play \in \players$ receives only the realized value of their observable, known as \emph{bandit} feedback \cite{SS11}.
%At this point, we weaken the feedback assumption even further and suppose that each player $\play \in \players$ receives only the realized value of their observable.
%As described in \eqref{eq:prob-density}, each outcome $\outcome_\run \in \outcomes$ of the \ac{POVM} is occurred with probability $\pdist_{\outcome}(\curr)$ under the strategy profile $\curr$. Thus, player $\play \in \players$ observes only the scalar value $\payobs_{\play}(\outcome_\run) \in \R$ and needs to approximate the payoff gradient through this single observation. 
In this information constrained setting, the standard \eqref{eq:MMW} is replaced by  
\begin{equation}
\label{eq:B-MMW}
\tag{B-MMW}
\begin{aligned}
&\dmat_{\play,\run+1}  = \dmat_{\play,\run} + \step_\run\paysignal_{\play,\run}\\
&\denmat_{\play,\run+1}  = \frac{\exp(\dmat_{\play,\run+1})}{\trof*{\exp(\dmat_{\play,\run+1})}}
\end{aligned}
\end{equation}
where $\paysignal_{\play,\run}$ is an estimate of the payoff gradient of player $\play$ under $\curr$, and all other quantities as before.
Thus, the challenge lies in reconstructing the payoff gradient matrix out of scalar observations.

\subsection{A naive approach -- Importance-weighting techniques}
Inspired by results in classical finite games, a standard approach for constructing $\paysignal_{\play,\run}$ would be through the \acdef{IWE} \needref.
Briefly, assuming $\play \in \players$ plays the \emph{full-supported} mixed strategy $\strat_{\play,\run}$ in the probability simplex of the finite set of actions $\pures_\play = \{\pure_1,\dots,\pure_{\abs{\pures_\play}}\}$, the idea of the \ac{IWE} is to approximate the payoff gradient (a vector in this case), through 
\begin{equation}
\label{eq:IWE}
\tag{IWE}
\hat\signal_{\play\pure_{\play},\run}
    = \frac{\oneof{\est\pure_{\play,\run} = \pure_{\play}}}{\strat_{\play\pure_{\play},\run}}
    \est\pay_{\play,\run}
    \quad \text{for } \pure_\play \in \pures_\play
\end{equation}
where $\est\pure_{\play,\run}$ is sampled from $\strat_{\play,\run}$ and $\est\pay_{\play,\run}$ is the scalar-valued feedback of player $\play \in \players$.
[The assumption that $\strat_{\play,\run}$ has full support is only for technical reasons. In practice, it can be relaxed by using \ac{IWE} with explicit exploration -- see \needref for more details.]

Nevertheless, it is clear that this approach would fail in the quantum framework from the ground up, for two reasons. 
The first one stems from the fact that in the quantum regime there is a \emph{continuum} of pure states available to every player, unlike the classical finite games where there is only a \emph{finite} set of pure actions. 
Secondly, even after the realization of the pure states of the players, there is an inherent uncertainty and randomness due to the payoff-generating quantum process.
To tackle these issues, we will take advantage of the continuous game reformulation of the quantum games, and employ a \acdef{SPSA} method \cite{Spa92} for estimating the payoff gradient.
In the next section, we present how the \ac{SPSA} method can be utilized to construct an approximate gradient out of scalar observations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\Large\Kyriakos{Until Here!}}
%\clearpage
%A first relaxation of the full observation assumption would be to consider that each player $\play \in \players$ does not receive their individual payoff gradient, but rather a noisy version of it, $\paysignal_{\play,\run}$, satisfying the following statistical properties:
%\begin{align}
%\label{eq:stochastic-statistics}
%\exof{\paysignal_{\play,\run} \given \filter_\run} = \payfield_{\play}(\curr)
%\quad \text{and} \quad
%\exof{\dnorm{\paysignal_{\play,\run}}^2 \given \filter_\run} \leq \sigma^2
%\end{align}
%where $\sigma$ is a (non-random) constant, and $\filter_\run = \sigma(\init,\dots,\curr)$ is the natural filtration generated by the sequence of play. In light of \eqref{eq:stochastic-statistics}, we show that the \emph{ergodic-average} sequence of \eqref{eq:MMW}
%\begin{equation}
%\label{eq:ergodic}
%\ergodic_\run = \parens*{\frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{1,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}, \frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{2,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}}
%\end{equation}
%converges to \ac{NE} point with rate $\bigoh(1/\sqrt{\run})$. Formally, we have the following preliminary result.
%
%\begin{restatable}{theorem}{stochastic}
%\label{eq:stochastic}
%Consider a 2-player zero-sum quantum game, where each player follows \eqref{eq:MMW} with stochastic feedback, as per \eqref{eq:stochastic-statistics}, and learning-rate parameters $\step_\run \propto 1/\sqrt\run$ for $\run \in \N$. Then, the ergodic sequence of play \eqref{eq:ergodic} converges to a \ac{NE} point with rate $\bigoh(1/\sqrt{\run})$.
%%satisfying (i) $\sum_{\run = 1}^\infty \step_\run = \infty$, and (ii) $\sum_{\run = 1}^\infty \step_{\run}^2 < \infty$.
%%\begin{equation}
%%\sum_{\run = 1}^\infty \step_\run = \infty
%%\quad \text{and} \quad
%%\sum_{\run = 1}^\infty \step_{\run}^2 = \infty
%%\end{equation}
%\end{restatable}
%
%However, the assumption that players receive a noisy version of their individual payoff gradient is still a strong condition; in an online learning framework, it is more realistic to consider that players observe only the impact of the \emph{realized} outcome of their actions.
%In what follows, we consider the case where players observe only their realized payoff, \ie a single scalar value, known as \emph{bandit} feedback \cite{SS11}.
%This feedback model is widely used in online optimization and game-theoretic learning \needref and is known as \emph{bandit} feedback \cite{SS11}.
%The standard \ac{MMW} assumes full payoff observations, meaning that each player $\play \in \players$ receives at each stage $\run \in \N$ of the learning process their individual payoff gradient $\payfield_{\play}(\denmat_{\play,\run})$ \needref. 
%However, in an online learning framework, it is more realistic to consider that players observe only the impact of the \emph{realized} outcome of their actions.
%This feedback model is widely used in online optimization and game-theoretic learning \needref and is known as \emph{bandit} feedback \cite{SS11}.
%In this work, we drop the full payoff observation assumption and assume that each player $\play \in \players$ receives as feedback only the realized value of their observable, $\payobs_{\play}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In contrast to finite games with bandit feedback, where the standard approach for players to reconstruct their payoff vectors is through the \acdef{IWE} \needref, we assume that players employ a \acdef{SPSA} method introduced by \cite{Spa92}, which is described in detail next. 
%The reason for this stark difference between the classical and the quantum regime is that in the latter there is a \emph{continuum} of pure states available to every player, while in the former there is only a \emph{finite} set of pure actions. 

\subsection{Gradient estimation via finite-difference on the spectraplex}
To illustrate the intuition of the \ac{SPSA} method, consider, first, a 1-dimensional differentiable function $f:\R \to \R$ and a point $x \in \R$. Then, for error tolerance $\radius > 0$, a two-point estimate of the derivative of $f$ at $x$ is given by the expression
\begin{equation}
%\hat f_x= \frac{1}{\radius}f(x+\radius s) s
\hat f_x = \frac{f(x+\radius) - f(x-\radius)}{2\radius} 
\end{equation}
Going to higher dimensions, letting $f: \R^d \to \R$ be a smooth function, $\{e_1,\dots,e_d \}$ be the standard basis of $\R^d$ and $s$ drawn from $\{e_1,\dots,e_d \}$ uniformly at random, the estimator
\begin{equation}
\label{eq:2-point-dif}
\hat f_x = \frac{d}{2\radius}\bracks*{f(x+\radius s) - f(x-\radius s)} s
\end{equation}
is a $\bigoh(\radius)$-approximation of the gradient, \ie $\dnorm{\ex_s[\hat f_x] - \nabla f(x)} = \bigoh(\radius)$. This idea is the basis of the \ac{SPSA} method.

%In view of the above, drawing $s$  from $\{\pm e_1,\dots,\pm e_d \}$ instead of the standard basis set, the estimator
%where $s$ is drawn from $\{\pm1\}$ uniformly at random. Then, $\hat f_x$ is an estimator of the ``discrete derivative''
%\begin{equation}
%\label{eq:1-point-der}
%\ex[\hat f_x] = \frac{f(x+\radius) - f(x-\radius)}{2\radius} 
%\end{equation}
%Note, that the above estimator requires the evaluation of $f$ at a single point only, \ie $f(x+\radius)$ or $f(x+\radius)$. 
%\begin{equation}
%\label{eq:1-point-dif}
%\hat f_x = \frac{d}{\radius}f(x+\radius s) s
%\end{equation}
%is still a $\bigoh(\radius)$-approximation of the gradient, but requires the evaluation of $f$ at a \emph{single point only}; this is the essence of the \ac{SPSA} method.

%, \ie $f(x+\radius s)$ or $f(x+\radius s)$.
%\begin{remark}
%For the rest of the section, we focus on player $\play$ and drop the indices altogether, for notational convenience.
%\end{remark}
%\vspace{-0.5em}
In order to utilize this type of estimator for a function over the set of density matrices $\denmats$ in $\herm[\vdim]$, we need to ensure two things: \textit{(i)} the feasibility of the \emph{sampling direction}, and \textit{(ii)} the feasibility of the \emph{evaluation point}. The first caveat is due to the fact that the set of the density matrices forms a lower dimensional manifold in the set of Hermitian operators, and therefore, not all directions from a base of $\herm[\vdim]$ are feasible. The second one is due to the fact that $\denmats$ is bounded, thus, even if the sampling direction is feasible, the evaluation point can lie outside the set $\denmats$. 
\vspace{-0.5em}

\para{Sampling Directions}
To account for the first restriction, we will construct an orthonormal basis of the affine hull of $\denmats_{0}$, where $\denmats_{0}= \setdef{\denmat \in\psd[\vdim]}{\tr\denmat = 0}$, and $\aff(\denmats_0)$ is the subspace of $\herm[\vdim]$ with all elements having trace equal to $0$, \ie $\aff(\denmats_{0}) = \setdef{\denmat \in\herm[\vdim]}{\tr\denmat = 0}$.
%\begin{equation}
%\label{eq:denmats-0}
%\denmats_{0}
%	= \setdef{\denmat \in\psd[\vdim]}{\tr\denmat = 0}
%\end{equation}
%and, $\aff(\denmats_0)$ is the subspace of $\herm[\vdim]$ with all elements having trace equal to $0$, \ie
%\begin{equation}
%\label{eq:aff-denmats-0}
%\aff(\denmats_{0})
%	= \setdef{\denmat \in\herm[\vdim]}{\tr\denmat = 0}
%\end{equation}
Note that if $\diagbasis \in \aff(\denmats_0)$ then for any $\denmat \in \herm[\vdim]$ it holds
\begin {enumerate*} [label=(\itshape\alph*\upshape)]
\item
$\denmat + \diagbasis \in \herm[\vdim]$, and
\item
$\trof{\denmat + \diagbasis} = \trof{\denmat}$.
\end {enumerate*} 

Denoting by $\diracmat_{k\ell} \in \herm[\vdim]$ the matrix with $1$ in the $(k,\ell)$-position and $0$'s everywhere else, it is easy to see that the set $\big\{\{\diracmat_{jj}\}_{j=1}^{\vdim} \{\nondiagbasis_{k\ell}\}_{k<\ell}, \{\tilde\nondiagbasis_{k\ell}\}_{k<\ell}\big\}$ is an orthonormal basis of $\herm[\vdim]$, where
\begin{align}
%\diagbasis_j & = \diracmat_{jj} \\
\nondiagbasis_{k\ell} = \frac{1}{\sqrt{2}}\diracmat_{k\ell} +  \frac{1}{\sqrt{2}}\diracmat_{k\ell} \quad & \text{and} \quad
\tilde\nondiagbasis_{k\ell} = \frac{i}{\sqrt{2}}\diracmat_{k\ell} - \frac{i}{\sqrt{2}}\diracmat_{k\ell}
\end{align}
for $1\leq k < \ell\leq\vdim$, where $i$ is the imaginary unit with $i^2 = -1$. The next proposition provides a basis for the subspace $\aff(\denmats_0)$, whose proof lies in the appendix.

\begin{restatable}{proposition}{basis}
\label{prop:basis}
Let $\diagbasis_j$ be defined as $\,\diagbasis_j = \frac{1}{\sqrt{j(j+1)}}\parens*{\diracmat_{11} + \dots + \diracmat_{jj} - j\diracmat_{(j+1)(j+1)}}\,$
%\begin{equation}
%\diagbasis_j = \frac{1}{\sqrt{j(j+1)}}\parens*{\diagbasis_1 + \dots + \diagbasis_j - j\diagbasis_{j+1}}
%\end{equation}
for $j = 1,\dots,\vdim-1$. 
Then, the set $\bvecs = \braces*{\{\diagbasis_j\}_{j=1}^{\vdim-1}, \{\nondiagbasis_{k\ell}\}_{k<\ell}, \{\tilde\nondiagbasis_{k\ell}\}_{k<\ell}}$ is an orthonormal basis of $\aff(\denmats_0)$.% and $\Dim \defeq \dim(\aff(\denmats_0)) = \defeq \vdim_{\play}^{2}-1$.% and $\dim(\aff(\denmats_0)) = \vdim^2 - 1$.
\end{restatable}

\para{Feasibility Adjustment}
After establishing an orthonormal basis for $\aff(\denmats_0)$ as per \cref{prop:basis}, we readily get that for any $\denmat \in \denmats$, any $\dir \in \dirs \defeq \big\{\{\pm\diagbasis_j\}_{j=1}^{\vdim-1}, \{\pm\nondiagbasis_{k\ell}\}_{k<\ell}, \{\pm\tilde\nondiagbasis_{k\ell}\}_{k<\ell}\big\}$ and $\radius > 0$, the point $\denmat + \radius\,\dir$ belongs to $\aff(\denmats)$.
However, depending on the value of the exploration parameter $\radius$ and the distance of $\denmat$ from the boundary of $\denmats$, the point $\denmat + \radius\dir \in \herm[\vdim]$ may fail to lie in $\denmats$ due to violation of the positive-semidefinite condition. Hence, we now treat the latter restriction, \ie the feasibility of the \emph{evaluation point}. 

To tackle this, the idea is to transfer the point $\denmat$ towards the interior of $\denmats$ and move along the sampled direction from there. For this, we need to find a reference point $\refmat \in \relint(\denmats)$ and a safety net $\safe >0$ such that $\refmat + \safe\dir \in \denmats$ for any $\dir \in \dirs$. Then, for $\radius \in (0,r)$, the point  
\begin{equation}
\label{eq:pivot}
\pivot \defeq \denmat + \frac{\radius}{\safe}(\refmat - \denmat)
\end{equation}
lies in $\relint(\denmats)$, and moving along $\dir \in \dirs$, we readily get a point in $\denmats$, since:
\begin{align}
\label{eq:perturbation}
\pivot + \radius\,\dir & = (1-\frac{\radius}{\safe})\denmat + \frac{\radius}{\safe}(\refmat + \safe\dir) \in \denmats
\end{align}
as a convex combination of two elements in $\denmats$. The following proposition provides an exact expression for $\refmat$ and $\safe$, whose proof lies in the appendix.

\begin{restatable}{proposition}{adjustment}
\label{prop:adjustment}
Let $\refmat \in \denmats$ be defined as $\refmat= \frac{1}{{\vdim}}\sum_{j = 1}^{\vdim}\diracmat_{jj}$.
%\begin{equation}
%\refmat= \frac{1}{{\vdim}}\sum_{j = 1}^{\vdim}\diracmat_{jj}
%\end{equation}
Then, for $\safe = \min\braces*{\frac{1}{\sqrt{\vdim(\vdim-1)}}, \frac{\sqrt{2}}{\vdim}}
$, it holds that $\refmat + \safe\dir \in \denmats$ for any direction $\dir \in \dirs$.
\end{restatable}
Applying the previous procedure to each player $\play \in \players$, and using \cref{prop:adjustment}, we obtain a reference point, $\refmat_\play$, and a safety net, $\safe_\play$, per player, which we will use in the sequel.
To illustrate how our method can be deployed, we begin with the simpler two-point payoff-based case, where each player may observe $\pay_{\play}(\denmat)$, and we defer the least informative bandit problem to the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Payoff-based and Bandit Learning in Zero-sum Quantum Games}

As noted before, we deploy a first, but of practical interest, relaxation of the full information setting, and assume each player $\play \in \players$ observes the mixed payoff $\pay_{\play}(\denmat)$ under the strategy profile $\denmat$.

\subsection{Payoff-based and learning in zero-sum quantum games}
In view of this, we provide the sequence of events for constructing the approximate payoff gradients, which serve as the intermediate steps between the two equations in \eqref{eq:B-MMW}.
Given state $\denmat_\run$ and sampling radius $\radius_\run$, the steps for generating $\paysignal_{\play,\run}$ for every player $\play \in \players$, proceed as follows:

\vspace{-2mm}
\begin{enumerate}[\textbf{Step} 1]
\itemsep0em 
\item
Draw a sampling direction $\dir_{\play,\run} \in \bvecs_{\play}$ and $\sign_{\play,\run} \in \{\pm 1\}$ uniformly at random, and, independently.
\item
\begin{enumerate}[\itshape (a)]
%\itemsep0em 
\item
Play $\,\pivot_{\play,\run} + \sign_{\play,\run}\,\radius_\run\,\dir_{\play,\run}\,$ and observe $\pay_{\play}(\pivot_{\run} + \sign_{\run}\radius_\run\dir_{\run})$.
\item
Play $\,\pivot_{\play,\run} - \sign_{\play,\run}\,\radius_\run\,\dir_{\play,\run}\,$ and observe $\pay_{\play}(\pivot_{\run} - \sign_{\run}\radius_\run\dir_{\run})$.
\end{enumerate}
%Simultaneously, all players query at points $\pivot_{\play,\run} + \sign_{\play,\run}\,\radius_\run\,\dir_{\play,\run}$ and $\pivot_{\play,\run} - \sign_{\play,\run}\,\radius_\run\,\dir_{\play,\run}$.
%\item
%Observe $\pay_{\play}(\pivot_{\run} + \sign_{\run}\radius_\run\dir_{\run})$ and $\pay_{\play}(\pivot_{\run} - \sign_{\run}\radius_\run\dir_{\run})$.
\item
Approximate $\payfield_{\play}(\denmat_\run)$  via the estimator:
\begin{equation}
\label{eq:Mix-SPSA}
\tag{2-PT}
\paysignal_{\play,\run} \defeq \frac{\Dim_{\play}}{2\radius_\run}\bracks*{\pay_{\play}(\pivot_{\run} + \sign_{\run}\radius_\run\dir_{\run}) - \pay_{\play}(\pivot_{\run} - \sign_{\run}\radius_\run\dir_{\run})}\,\sign_{\play,\run}\dir_{\play,\run}
\end{equation}
\end{enumerate}
where $\Dim_\play = \vdim_{\play}^{2}-1$ the dimension of $\herm[\vdim_{\play}]$, and $\Dim \defeq \max_{\play\in\players}\Dim_\play$. Letting $\filter_\run = \sigma(\init,\dots,\curr)$ be the natural filtration generated by the sequence of play, the \eqref{eq:Mix-SPSA} estimator enjoys the following statistical bounds.

\begin{restatable}{proposition}{MixStatistics}
\label{prop:Mix-SPSA-statistics}
The estimator \eqref{eq:Mix-SPSA} satisfies the following statistical properties:
\begin{equation}
\label{eq:Mix-SPSA-statistics}
\text{(i)}\quad
\dnorm*{\ex\bracks*{\paysignal_{\play,\run} \mid \filter_\run} - \payfield_\play(\denmat_\run)} \leq \frac{1}{2}\Dim_\play \smooth \nPlayers^{2}\radius_{\run}
\quad \text{and} \quad \text{(ii)}\quad
\ex\bracks*{\dnorm*{\paysignal_{\play,\run}}^2  \mid \filter_\run} \leq \Dim_{\play}^{2}\lips^{2}\nPlayers^{2}
\end{equation}
\end{restatable}
%
After establishing the statistical properties of \eqref{eq:Mix-SPSA}, we are ready to present our theorem on the convergence of the time-average sequence, $\ergodic_{\nRuns}$,
%\begin{equation}
%\label{eq:timeavg}
%\ergodic_{\playone,\nRuns} = \frac{1}{\nRuns}\sum_{\run = 1}^\nRuns \denmat_{\playone,\run}
%\quad\text{and}\quad
%\ergodic_{\playtwo,\nRuns} = \frac{1}{\nRuns}\sum_{\run = 1}^\nRuns \denmat_{\playtwo,\run}
%\end{equation}
of the \ac{MMW} with mixed-payoff feedback for a zero-sum quantum game. 

\begin{restatable}{theorem}{mixedzero}
\label{thm:mixed-zero}
Consider a 2-player zero-sum quantum game, where each player follows \eqref{eq:B-MMW} with mixed-payoff feedback, as per \eqref{eq:Mix-SPSA}, for $\nRuns$ epochs with $\step_\run = \step$  and $\radius_\run = \radius$ for $\run = 1,\dots,\nRuns$, and $\dmat_1 = 0$. Then, the time-average sequence of play $\ergodic_{\nRuns}$ enjoys the following bound:
\begin{align}
\exof*{\gap_{\loss}(\ergodic_{\nRuns})}
& \leq \frac{\hmax}{\step\nRuns} +  8\Dim^2\lips^2 \step+ 16\Dim\smooth\radius
\end{align}
Specifically, for $\step = \sqrt{\frac{\hmax}{8\nRuns\Dim^2\lips^2}}$ and $\radius = \sqrt{\frac{\lips^2 \hmax}{8\smooth^2\nRuns}}$, we obtain:
\begin{align}
\exof*{\gap_{\loss}(\ergodic_{\nRuns})}
& \leq \frac{8\sqrt{2\hmax}\Dim\lips}{\sqrt\nRuns}
\end{align}
%and for any $\eps >0$, we get $\,\exof*{\gap_{\loss}(\ergodic_{\playone,\run},\ergodic_{\playtwo,\run})} \leq \eps\,$ for $\nRuns \geq \ceil*{128\Dim^2\lips^2\hmax/\eps^2}$ epochs.
\end{restatable}

\subsection{Bandit learning in zero-sum quantum games}
At this point, we are ready to present the \ac{MMW} with minimal information assumptions when players observe only the impact of the realized outcome, \ie the value of their payoff observable after the measurement that eliminates the quantum uncertainty.
As described in \eqref{eq:prob-density}, each outcome $\outcome_\run \in \outcomes$ of the \ac{POVM} is occurred with probability $\pdist_{\outcome}(\curr)$ under the strategy profile $\curr$. Thus, player $\play \in \players$ observes only the scalar value $\payobs_{\play}(\outcome_\run) \in \R$ and needs to approximate the payoff gradient through this single observation. 
\vspace{-2mm}
\begin{enumerate}[\textbf{Step} 1]
\itemsep0em 
\item
Draw a sampling direction $\dir_{\play,\run} \in \bvecs_{\play}^{\pm}$ uniformly at random.
\item
Simultaneously, all players query at point $\pivot_{\play,\run} + \radius_\run\,\dir_{\play,\run}$.
%Instead of moving towards $\dir_{\play,\run}$ form $\denmat_{\play,\run}$, \ie playing $\denmat_{\play,\run} + \radius_\run\dir_{\play,\run}$, perform the feasibility adjustment as per \eqref{eq:pivot},
%and play $\hat\denmat_{\play,\run} \defeq (1-{\radius_\run}/{\safe_\play})\denmat_{\play,\run} + {\radius_\run}/{\safe_\play}\cdot(\refmat_\play + \safe_\play\dir_{\play,\run})$ to ensure the feasibility of the evaluation point.
\item
Observe $\payobs_{\play}(\outcome_\run)$.
%\item
%Under $\hat\denmat_\run$, each $\outcome \in \outcomes$ is occurred with probability $\pdist_{\outcome}(\hat\denmat_\run)$. 
%Player $\play \in \players$ observes $\payobs_{\play}(\outcome_\run)$, where $\outcome_\run$ is the random outcome.
\item
Approximate $\payfield_{\play}(\denmat_\run)$  via the estimator:
\begin{equation}
\label{eq:B-SPSA}
\tag{B-SPSA}
\paysignal_{\play,\run} \defeq \frac{\Dim_{\play}}{\radius_\run}\payobs_{\play}(\outcome_\run)\,\dir_{\play,\run}
\end{equation}
\end{enumerate}
Finally, putting all the pieces together, we provide the pseudocode implementation of the \ac{MMW} with bandit feedback for quantum games in \cref{alg:B-SPSA}.
\begin{algorithm}[H]
\caption{MMW with bandit feedback}
\label{alg:B-SPSA}
\begin{algorithmic}[1]
	\State
	Input: $\dmat_1$, safety net $\safe_\play$ and reference point $\refmat_{\play}$ for $\play \in \players$ , step-size $\step_\run$, exploration parameter $\radius_\run$	
	\For{$\run = 1,2,\dots$ simultaneously for all players $\play \in \players$}
		\State
		Obtain $\denmat_{\play,\run}  = {\exp(\dmat_{\play,\run})}/{\trof{\exp(\dmat_{\play,\run})}}$.
		\State
		Sample $\dir_{\play,\run}$ uniformly from $\bvecs_{\play}^{\pm}$.
		\State
		Play strategy $\pivot_{\play,\run} + \radius_{\run} \dir_{\play,\run}$.%\defeq (1-{\radius_\run}/{\safe_\play})\denmat_{\play,\run} + {\radius_\run}/{\safe_\play}\cdot(\refmat_\play + \safe_\play\dir_{\play,\run})$		
		\State
		Observe $\payobs_{\play}(\outcome_\run)$.
		\State
		Estimate $\paysignal_{\play,\run} \defeq {\Dim_\play}/{\radius_\run} \cdot \payobs_{\play}(\outcome_\run)\dir_{\play,\run}$.
		\State
		Update $\dmat_{\play,\run+1}  = \dmat_{\play,\run} + \step_\run\paysignal_{\play,\run}$.
		%Update $\denmat_{\play,\run+1} \leftarrow \denmat_{\play,\run}\exp(\step_\run\paysignal_{\play,\run})/\trof*{ \denmat_{\play,\run}\exp(\step_\run\paysignal_{\play,\run})}$.
	\EndFor
\end{algorithmic}
\end{algorithm}

\begin{restatable}{proposition}{statistics}
\label{prop:B-SPSA-statistics}
The estimator \eqref{eq:B-SPSA} satisfies the following statistical properties:
\begin{equation}
\label{eq:Mix-SPSA-statistics}
\text{(i)}\quad
\dnorm*{\ex\bracks*{\paysignal_{\play,\run} \mid \filter_\run} - \payfield_\play(\denmat_\run)} \leq \frac{1}{2}\Dim_\play \smooth \nPlayers^{2}\radius_{\run} % \bigoh(\radius_\run)
\quad \text{and} \quad \text{(ii)}\quad
\ex\bracks*{\dnorm*{\paysignal_{\play,\run}}^2  \mid \filter_\run} \leq \frac{\Dim_{\play}^{2}\bound^{2}}{\radius_\run^2} %= \bigoh(1/\radius_{\run}^{2})
\end{equation}
\end{restatable}

\begin{restatable}{theorem}{banditzero}
\label{thm:bandit-zero}
Consider a 2-player zero-sum quantum game, where each player follows \eqref{eq:B-MMW} with bandit feedback, as per \cref{alg:B-SPSA}, for $\nRuns$ epochs with $\step_\run = \step$  and $\radius_\run = \radius$ for $\run = 1,\dots,\nRuns$, and $\dmat_1 = 0$. Then, the time-average sequence of play $\ergodic_{\nRuns}$ enjoys the following bound:
\begin{align}
\exof*{\gap_{\loss}(\ergodic_{\nRuns})}
& \leq \frac{\hmax}{\step\nRuns} + \frac{2\Dim^2\bound^2\step}{\strong\radius^2} + 16\Dim\smooth\radius
\end{align}
Specifically, for $\step = \parens*{\frac{\hmax}{2\nRuns}}^{3/4} \frac{1}{2\Dim\sqrt{\bound\smooth}}$ and $\radius = \parens*{\frac{\hmax}{2\nRuns}}^{1/4}\sqrt{\frac{\bound}{4\smooth}}$, we obtain:
\begin{align}
\exof*{\gap_{\loss}(\ergodic_{\nRuns})}
& \leq \frac{2^{3/4}\,8\Dim\sqrt{\bound\smooth}\hmax^{1/4}}{\nRuns^{1/4}} 
\end{align}
%and for any $\eps >0$, we get $\,\exof*{\gap_{\loss}(\ergodic_{\playone,\run},\ergodic_{\playtwo,\run})} \leq \eps\,$ for $\nRuns \geq \ceil*{2^{15}\Dim^{4}\bound^2\smooth^2\hmax/\eps^4}$ epochs.
\end{restatable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Bandit Learning in General Quantum Games}

Going beyond the setup of two-player zero-sum games, we consider a general $\nPlayers$-player quantum game, where a key characteristic to keep in mind is that it may admits several Nash equilibria.
Therefore, it is not reasonable to expect a global convergence result that applies to all games.
In light of this, we focus on quantum states that satisfy a certain property known as \acdef{VS}.

The \eqref{eq:VS} condition can be seen as the analog of a \emph{first-order stationarity} condition in the context of continuous optimization, or
as an equilibrium refinement in the spirit of the seminal concept of \emph{evolutionary stability} \cite{MP73,May82}.
In the setting of classical finite games, the notion of variational stability is tightly related to the strict Nash equilibria.
Precisely, a strategy profile is variationally stable if and only if it is a strict \ac{NE}. % \cite{GVM21}.
In turn, \cite{GVM21} showed that \eqref{eq:VS} property fully characterizes the points that are stochastically asymptotically stable, \ie points that attract all nearby points with arbitrarily high probability, under the $\acdef{FTRL}$ framework, which encloses the \acdef{EW} algorithm as a special case.
%In turn, \cite{GVM21} showed that only variationally stable points can be attracting under the $\acdef{FTRL}$ framework, which encloses the \acdef{EW} algorithm as a special case.
Moving to the quantum regime, \cite{LMB23} showed that only variationally stable states can be attracting under \acdef{RD}, and as a result, the \eqref{eq:VS} condition is the only hope for getting \emph{last-iterate} convergence results in general quantum games.
In light of the above, \cref{thm:banditgeneral} serves as a first algorithmic justification of the full information, continuous-time result of \cite{LMB23}. 
Formally, the \eqref{eq:VS} property is defined as follows.

%The \eqref{eq:VS} condition can be seen as a \emph{first-order stationarity} condition in the context of continuous optimization, or
%as an equilibrium refinement in the spirit of the seminal concept of \emph{evolutionary stability} \cite{MP73,May82}.
%Formally, the \eqref{eq:VS} property is defined as follows.
\begin{definition}
\label{def:VS}
We say that $\eq\in\denmats$ is \emph{\textpar{locally} variationally stable} if there exists a neighborhood $\pnhd$ of $\eq$ in $\denmats$ such that
\begin{equation}
\label{eq:VS}
\tag{VS}
\trof{\payfield(\denmat) (\denmat - \eq)}
	< 0
	\quad
	\text{for all $\denmat\in\pnhd\exclude{\eq}$}.
\end{equation}
\end{definition}

In words, \eqref{eq:VS} implies that the payoff gradients, $\payfield(\denmat)$, point towards $\eq$ in a neighborhood of the latter point, \ie $\eq$ strictly dominates all other strategies $\denmat$ nearby.
As a consequence, the \eqref{eq:VS} condition allows us to consider last-iterate results, due to a ``consistent drift'' on the sequence of play towards the variationally stable point $\eq$ within a neighborhood of the latter.

Note that the last-iterate convergence serves as a stronger notion of convergence, as it refers to the \emph{actual sequence-of-play}, $\denmat_\run$, and not the \emph{time-averaged} one, $\ergodic_\run$, as in the case of zero-sum games. % , which serves as a stronger notion of convergence than the time-averaged one.
%It is important to highlight here that the above result refers to the \emph{actual sequence-of-play}, $\denmat_\run$, and not the \emph{time-averaged} one, as in the case of zero-sum games.
Importantly, the time-averaged results do not provide any convergence guarantee for the actual strategy profile being followed by the players. 
However, in cases that require to track the trajectory of the system, or the actual day-to-day reward, this mode of convergence provides justification and guarantees for the true sequence of events.

In view of the above, unlike the time-averaged sequence where the impact of noise is averaged out, here a single unfavorable realization of the noise can move the process outside the region of attraction, ruining the convergence, altogether. Therefore, to achieve asymptotic convergence it requires a more careful tuning of the step-size $\step_\run$ and the exploration parameter $\radius_\run$. 
Specifically, we need to consider step-size and exploration parameters small enough such that the impact of noise vanishes out, but at the same time large enough so that convergence is achieved.  
For this reason, we need to consider diminishing step-size and exploration schedules, in contrast to the previous cases. 
Formally, our result is stated as follows.

%Therefore, the analysis is much more delicate, leveraging results from martingale convergence theory.
\begin{restatable}{theorem}{banditgeneral}
\label{thm:banditgeneral}
Consider a $\nPlayers$-player quantum game and let $\eq$ be a variational stable point, as per \eqref{eq:VS}. Fix some confidence level $\conf \in (0,1)$. 
If each player follows \eqref{eq:MMW} with bandit feedback, as per \cref{alg:B-SPSA}, with learning-rate and sampling radius parameters satisfying
\begin{equation}
\label{eq:hyperparameters-general}
\text{(i)}\quad
\sum_{\run = 1}^\infty \step_\run = \infty,
\quad \text{(ii)}\quad
\sum_{\run = 1}^\infty \step_\run \radius_\run < \infty,
\quad\text{and} \quad \text{(ii)}\quad
\sum_{\run = 1}^\infty \step_{\run}^2/\radius_{\run}^2 < \infty
\end{equation}
then, there exists a neighborhood $\nhd$ of $\eq$ in $\denmats$ such that
\begin{equation}
\probof*{\lim_{\run \to \infty} \curr = \eq \given \init \in \nhd} \geq 1-\conf
\end{equation} 
\end{restatable}

%Precisely, the \eqref{eq:VS} condition allows us to consider \emph{last-iterate} convergence results, due to a consistent drift on the sequence of play towards the variationally stable point $\eq$ within a neighborhood of the latter. 
%Unlike the time-averaged sequence, where the impact of noise is averaged out, here a single unfavorable realization of the noise can  move the process outside the region of attraction, ruining the convergence, altogether. Therefore, the analysis is much more delicate, leveraging results from martingale convergence theory.
%The time-average does not provide any convergence guarantee for the actual sequence of play. However, in many cases it is important to track to and provide for the actual sequence of events.


%\begin {enumerate*} [label=(\itshape i\upshape)] 
%\item 
%$\diagbasis_i = \diracmat_{ii}$,
%\item
%$\nondiagbasis_{ij} = \frac{1}{\sqrt{2}}\diracmat_{ij} +  \frac{1}{\sqrt{2}}\diracmat_{ji}$, and
%\item 
%$\tilde\nondiagbasis_{ij} = \frac{i}{\sqrt{2}}\diracmat_{ij} - \frac{i}{\sqrt{2}}\diracmat_{ji}$
%\end{enumerate*}
%Note, that the above estimate requires the evaluation of $f$ at two points, $f(x+\radius)$ and $f(x+\radius)$. To further reduce to single-point approximation, one can randomize the point of evaluation between $x\pm\radius$. More rigorously, letting $s $ be ${\pm 1}$ uniformly at random, the quantity is an unbiased estimator of \eqref{eq:2-point-der}. 

==> Body/Discussion.tex <==
%----------------------------------------------------------------------
%%% DISCUSSION
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


This is the discussion section.

==> Body/Introduction_old_backup.tex <==
%----------------------------------------------------------------------
%%% INTRODUCTION
%----------------------------------------------------------------------
% !TEX root = ../Main.tex
The integration of quantum information theory into computer science and machine learning \cite{Pre18,AABB+19,ZWDC+20} has the potential to transform the field by providing faster and more efficient computing resources, new encryption and security protocols, and improved machine learning algorithms, enabling advancements in areas such as quantum cryptography, shadow tomography, QGAN, and adversarial learning \cite{Aar20,DK18,CHL19,LW18}.
%The emergence of quantum information theory and its related concept of "quantum advantage" \cite{Pre18,AABB+19,ZWDC+20} have had a significant impact on computer science and machine learning, enabling advancements in areas such as quantum cryptography, shadow tomography, QGAN, and adversarial learning \cite{Aar20,DK18,CHL19,LW18}.
Training an autonomous vehicle model in less than 200 seconds, Google's "Sycamore" 54-qubit processor showcases this  "quantum advantage" \cite{AABB+19},
which stems from the ability of quantum computers to prepare superpositions of qubits.
%potential of quantum computing to greatly accelerate the development of artificial intelligence algorithms and models.
%Training an autonomous vehicle model in less than 200 seconds, Google's "Sycamore" 54-qubit processor showcases the potential of quantum computing to greatly accelerate the development of artificial intelligence algorithms and models \cite{AABB+19}. 
%These advantages stem from the ability of quantum computers to prepare superpositions of qubits. % \ie binary-state quantum systems. 
%This is due to the advantages offered by quantum-based computing, which stem from the ability to prepare superpositions of qubits, \ie binary-state quantum systems. 
In contrast, classical computers are limited by their binary alphabet and memory structure, since classical bits cannot exist in superposition. 

Deploying such models within a multi-agent context, such as the utilization of QGANs or autonomous vehicles, leads to a significant transformation compared to classical non-cooperative environments. 
This shift primarily arises due to the inherent properties of quantum systems, namely the decoherence and entanglement principle. %, with no classical analog. 
Specifically, these quantum notions enable quantum players to possess an edge over "classical" ones, attaining greater payoffs than would be achievable \cite{Mey99,EWL99}.
%Specifically, these quantum notions enable quantum players to possess an edge over "classical" ones, attaining greater payoffs at equilibrium than would be achievable \cite{Mey99,EWL99}.
This phenomenon occurs due to the disparity in probabilistic mixing between the quantum and classical domains. 
Unlike classical games, where a mixed strategy is a probabilistic mixture of the underlying pure strategies, quantum games utilize mixed states, which represent probabilistic mixtures of quantum projectors. % associated with each constituent state. 
As a consequence, a mixed quantum state can yield payoffs that cannot be expressed as a convex combination of classical pure strategies. 

%This phenomenon occurs due to the disparity in probabilistic mixing between the quantum and classical domains. 
%In classical games, a mixed strategy involves a probabilistic  mixture of the underlying pure strategies. In contrast, quantum games utilize mixed states, which represent probabilistic mixtures of quantum projectors associated with each constituent state. 
%As a consequence, a mixed quantum state can yield payoffs that cannot be expressed as a convex combination of classical pure strategies. 

In light of this, learning in quantum games have drawn significant attention in recent years. The most widely used framework for learning quantum states is the \acdef{MMW} algorithm \cite{JW09,JPS22,LPSV23,ACHK+18,chen2022adaptive}.
Introduced by \citet{TRW05},  \ac{MMW}  can be viewed as the matrix analog of the standard Hedge / EXP3 methods in single-agent learning \cite{Vov90, LW94, ACBFS95}. 
In the context of quantum games, \citet{JW09} studied the problem learning a \acdef{NE} in two-player zero-sum quantum games, achieving $\bigoh(1/\sqrt{\nRuns})$-ergodic convergence. % of the \ac{MMW} to the set of Nash equilibria in two-player zero-sum quantum games, which .
This result remains the tightest known bound for Nash equilibrium learning in 2-player zero-sum quantum games, to the best of our knowledge.
Following the  work of \cite{JW09}, \citet{JPS22} studied its continuous-time analog, namely \acdef{QRD}, in quantum zero-sum games, showing that the dynamics exhibit the Poincaré recurrence property.
Going beyond the class of quantum zero-sum games, \cite{LMB23} extended this result introducing the so-called \acdef{FTQL} dynamics, a quantum analog of the well-studied \acdef{FTRL} framework in classical finite games \cite{SS07,SSS06}, showing a quantum analog of the classical ``folk theorem'' of evolutionary game theory \cite{Cre03,HS03}.
In a similar line of work, \citet{LPSV23} studied the continuous-time, \ac{QRD}, and discrete-time, \ac{MMW}, dynamics in quantum potential games.
All the previous works, assume full information, \ie players have access on their individual gradients \textendash\ which, among others, might imply that they have full knowledge of the game.
However, this condition is rarely met in an online game-theoretic learning framework.
In this work, we relax precisely this assumption and develop a payoff-based, gradient-free variant of \ac{MMW}. 
\vspace{-3mm}
\para{Our contributions}

We develop the first learning framework with minimal information in quantum games, namely a payoff-based variant of the \ac{MMW}.
In contrast to classical finite games, where a standard approach for estimating the payoff gradient relies on importance-weighting techniques,
this method would fail in the quantum setup from the ground up, for two reasons. 
Firstly, there is a \emph{continuum} of pure states available to every player, unlike the classical finite games where there is only a \emph{finite} set of pure actions. 
Secondly, even after the realization of the pure states of the players, there is an inherent uncertainty and randomness due to the payoff-generating quantum process, with no classical counterpart.
Instead, we utilize the continuous game reformulation of the quantum games, and employ techniques from bandit convex optimization for estimating the payoff gradient.
In light of this, we develop a 2-point-estimation learning algorithm that achieves $\bigoh(1/\sqrt{\nRuns})$-ergodic convergence to the set of Nash equilibria in two-player zero-sum quantum games, matching the rate of the full information \ac{MMW} in \cite{JW09}.
Reducing the feedback available to players even further, where they observe only their individual realized payoffs, \ie a single scalar value, we design a learning procedure that converges to the set of \ac{NE} at a rate of $\bigoh({\nRuns}^{-1/4})$.
Finally, we provide the first local convergence guarantee in the context of $\nPlayers$-player general quantum games under some variational stability assumptions.






==> Body/Model_old.tex <==
%----------------------------------------------------------------------
%%% MODEL
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


The \acdef{MMW} algorithm is the most commonly utilized method for computing Nash equilibria in quantum games \needref. Formally, it is described by the following discrete-time dynamical system
\begin{equation}
\label{eq:MMW}
\tag{MMW}
\begin{aligned}
\denmat_{\play,\run} & = \frac{\exp(\dmat_{\play,\run})}{\trof*{\exp(\dmat_{\play,\run})}} \\
\dmat_{\play,\run+1} & = \dmat_{\play,\run} + \step_\run\payfield_{\play}(\curr)
\end{aligned}
\end{equation}
%\begin{equation}
%\label{eq:MMW}
%\tag{MMW}
%\begin{aligned}
%\denmat_{\play,\run+1} = \frac{\denmat_{\play,\run}\exp(\step_\run\payfield_{\play}(\curr))}{\trof*{ \denmat_{\play,\run}\exp(\step_\run\payfield_{\play}(\curr))}}
%\end{aligned}
%\end{equation}
%for $\run = 1,2,\dots$, where $\curr = (\denmat_{1,\run},\dots,\denmat_{\nPlayers,\run})$ is the strategy profile of the players at step $\run$ of the algorithm, $\step_\run$ is the learning-rate parameter, and $\paysignal_{\play,\run}$ is an estimate of the payoff gradient of player $\play$ under $\curr$.
for  $\play \in \players$ and $\run = 1,2,\dots$, where $\curr = (\denmat_{\playone,\run},\denmat_{\playtwo,\run})$ is the strategy profile of the players at step $\run$ of the algorithm, $\step_\run$ is the learning-rate parameter, and $\payfield_{\play}(\curr)$ is the payoff gradient of player $\play \in \players$ under $\curr$.
It is important to highlight that the vanilla \ac{MMW} algorithm assumes \emph{full-payoff observations}, in the sense that each player $\play \in \players$ receives at each stage $\run \in \N$ of the learning process their individual payoff gradient, $\payfield_{\play}(\curr)$, as indicated by the second equation in \eqref{eq:MMW}.

\citet{JW09} study the problem of computing an $\eps$-\ac{NE} in a 2-player quantum zero-sum game. Specifically, it is proven that the \emph{time-average} sequence of play of \eqref{eq:MMW}
%\begin{equation}
%\label{eq:ergodic}
%\ergodic_\run = \parens*{\frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{1,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}, \frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{2,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}}
%\end{equation}
converges to a \ac{NE} point with rate $\bigoh(1/\sqrt{\nRuns})$ after $\nRuns$ epochs, in the following sense.
\begin{theorem}[Informal, {\citet[Theorem~1]{JW09}}]
Consider a 2-player zero-sum quantum game, where each player follows \eqref{eq:MMW} for $\nRuns$ epochs with $\step_\run = \step = \Theta(1/\sqrt{\nRuns})$ for $\run = 1,\dots,\nRuns$. Then, the time-average sequence of play
\begin{equation}
\label{eq:ergodic}
\ergodic_{\playone,\nRuns} = \frac{1}{\nRuns}\sum_{\run = 1}^\nRuns \denmat_{\playone,\run}
\quad\text{and}\quad
\ergodic_{\playtwo,\nRuns} = \frac{1}{\nRuns}\sum_{\run = 1}^\nRuns \denmat_{\playtwo,\run}
\end{equation}
enjoys the following bound
\begin{equation}
\max_{\denmat_{\playone} \in \denmats_{\playone}} \loss(\denmat_{\playone},\ergodic_{\playtwo,\nRuns}) - \alpha/\sqrt{\nRuns} \leq
\loss(\ergodic_{\playone,\nRuns},\ergodic_{\playtwo,\nRuns}) \leq 
\min_{\denmat_{\playtwo} \in \denmats_{\playtwo}} \loss(\ergodic_{\playone,\nRuns},\denmat_{\playtwo}) + \alpha/\sqrt{\nRuns}
\end{equation}
for some constant $\alpha > 0$.
\end{theorem}

The above result remains the state-of-the-art in computing a \ac{NE} point in a zero-sum quantum game, to the best of our knowledge. 
However, the assumption that players receive their individual payoff gradient is very strong. In what follows, we extend this result twofolds.
On the one hand, we relax the full payoff observation assumption and go to the other extreme, considering the case where players observe only their realized payoff value. 
On the other hand, we expand our methods beyond the class of zero-sum games, to general $\nPlayers$-player quantum games under certain variational stability conditions.
%and what are the inherent difficulties of this.
%meaning that the estimates of the payoff gradients are exact throughout the execution of the learning process, \ie  $\paysignal_{\play,\run} = \payfield_{\play}(\curr)$ for all $\play \in \players$ and $\run \in \N$. 
%In the sequel, we examine how we can relax this assumption and what are the inherent difficulties of this.
%\citet{JW09} study the problem of computing an $\eps$-\ac{NE} in a 2-player quantum zero-sum game. Specifically, it is proven that the \emph{time-averaged} sequence of play of \eqref{eq:MMW} converges to a \ac{NE} point with rate $\bigoh(1/\sqrt{\run})$, where $\run$ is the time-step of the algorithm.
%However, the aformentioned result assumes full-payoff observations, in the sense that each player $\play \in \players$ receives at each stage $\run \in \N$ of the learning process their individual payoff gradient $\payfield_{\play}(\curr)$, as described before. %, which is not realistic in an online learning setting.
%is an approximate payoff matrix, \ie an estimate of $\payfield_{\play}(\denmat_{\play,\run})$ based on the feedback players receive.
%In what follows, we analyze the feedback form players receive and how it can be used to construct an approximate payoff matrix, $\paysignal_{\play,\run}$.

\section{The Bandit-\ac{MMW} Algorithm} 

In an online learning framework, it is more realistic to consider that players observe only the impact of the \emph{realized} outcome of their actions, \ie
each player $\play \in \players$ receives only the realized value of their observable, known as \emph{bandit} feedback \cite{SS11}.
%At this point, we weaken the feedback assumption even further and suppose that each player $\play \in \players$ receives only the realized value of their observable.
As described in \eqref{eq:prob-density}, each outcome $\outcome_\run \in \outcomes$ of the \ac{POVM} is occurred with probability $\pdist_{\outcome}(\curr)$ under the strategy profile $\curr$. Thus, player $\play \in \players$ observes only the scalar value $\payobs_{\play}(\outcome_\run) \in \R$ and needs to approximate the payoff gradient through this single observation. In this information constrained setting, the standard \eqref{eq:MMW} described before is replaced by  
\begin{equation}
\label{eq:B-MMW}
\tag{B-MMW}
\begin{aligned}
\denmat_{\play,\run} & = \frac{\exp(\dmat_{\play,\run})}{\trof*{\exp(\dmat_{\play,\run})}} \\
\dmat_{\play,\run+1} & = \dmat_{\play,\run} + \step_\run\paysignal_{\play,\run}
\end{aligned}
\end{equation}
where $\paysignal_{\play,\run}$ is an estimate of the payoff gradient of player $\play$ under $\curr$, and all other quantities as before.
Thus, the challenge lies in reconstructing the payoff gradient matrix out of a scalar observation.

\para{A naive approach -- Importance-weighting techniques}
Inspired by results in classical finite games, a standard approach for constructing $\paysignal_{\play,\run}$ would be through the \acdef{IWE} \needref.
Briefly, assuming $\play \in \players$ plays the \emph{full-supported} mixed strategy $\strat_{\play,\run}$ in the probability simplex of the finite set of actions $\pures_\play = \{\pure_1,\dots,\pure_{\abs{\pures_\play}}\}$, the idea of the \ac{IWE} is to approximate the payoff gradient (a vector in this case), through 
\begin{equation}
\label{eq:IWE}
\tag{IWE}
\hat\signal_{\play\pure_{\play},\run}
    = \frac{\oneof{\est\pure_{\play,\run} = \pure_{\play}}}{\strat_{\play\pure_{\play},\run}}
    \est\pay_{\play,\run}
    \quad \text{for } \pure_\play \in \pures_\play
\end{equation}
where $\est\pure_{\play,\run}$ is sampled from $\strat_{\play,\run}$ and $\est\pay_{\play,\run}$ is the scalar-valued feedback of player $\play \in \players$.
[The assumption that $\strat_{\play,\run}$ has full support is only for technical reasons. In practice, it can be relaxed by using \ac{IWE} with explicit exploration -- see \needref for more details.]

Nevertheless, it is clear that this approach would fail in the quantum framework from the ground up, for two reasons. 
The first one stems from the fact that in the quantum regime there is a \emph{continuum} of pure states available to every player, unlike the classical finite games where there is only a \emph{finite} set of pure actions. 
Secondly, even after the realization of the pure states of the players, there is quantum uncertainty and randomness due to the payoff-generating process.
To tackle these issues, we will take advantage of the continuous game reformulation of the quantum games, and employ a \acdef{SPSA} method \cite{Spa92} for estimating the payoff gradient.
In the next section, we present how the \ac{SPSA} method can be utilized to construct an approximate gradient out of a scalar observation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\Large\Kyriakos{Until Here!}}
%\clearpage
%A first relaxation of the full observation assumption would be to consider that each player $\play \in \players$ does not receive their individual payoff gradient, but rather a noisy version of it, $\paysignal_{\play,\run}$, satisfying the following statistical properties:
%\begin{align}
%\label{eq:stochastic-statistics}
%\exof{\paysignal_{\play,\run} \given \filter_\run} = \payfield_{\play}(\curr)
%\quad \text{and} \quad
%\exof{\dnorm{\paysignal_{\play,\run}}^2 \given \filter_\run} \leq \sigma^2
%\end{align}
%where $\sigma$ is a (non-random) constant, and $\filter_\run = \sigma(\init,\dots,\curr)$ is the natural filtration generated by the sequence of play. In light of \eqref{eq:stochastic-statistics}, we show that the \emph{ergodic-average} sequence of \eqref{eq:MMW}
%\begin{equation}
%\label{eq:ergodic}
%\ergodic_\run = \parens*{\frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{1,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}, \frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{2,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}}
%\end{equation}
%converges to \ac{NE} point with rate $\bigoh(1/\sqrt{\run})$. Formally, we have the following preliminary result.
%
%\begin{restatable}{theorem}{stochastic}
%\label{eq:stochastic}
%Consider a 2-player zero-sum quantum game, where each player follows \eqref{eq:MMW} with stochastic feedback, as per \eqref{eq:stochastic-statistics}, and learning-rate parameters $\step_\run \propto 1/\sqrt\run$ for $\run \in \N$. Then, the ergodic sequence of play \eqref{eq:ergodic} converges to a \ac{NE} point with rate $\bigoh(1/\sqrt{\run})$.
%%satisfying (i) $\sum_{\run = 1}^\infty \step_\run = \infty$, and (ii) $\sum_{\run = 1}^\infty \step_{\run}^2 < \infty$.
%%\begin{equation}
%%\sum_{\run = 1}^\infty \step_\run = \infty
%%\quad \text{and} \quad
%%\sum_{\run = 1}^\infty \step_{\run}^2 = \infty
%%\end{equation}
%\end{restatable}
%
%However, the assumption that players receive a noisy version of their individual payoff gradient is still a strong condition; in an online learning framework, it is more realistic to consider that players observe only the impact of the \emph{realized} outcome of their actions.
%In what follows, we consider the case where players observe only their realized payoff, \ie a single scalar value, known as \emph{bandit} feedback \cite{SS11}.
%This feedback model is widely used in online optimization and game-theoretic learning \needref and is known as \emph{bandit} feedback \cite{SS11}.
%The standard \ac{MMW} assumes full payoff observations, meaning that each player $\play \in \players$ receives at each stage $\run \in \N$ of the learning process their individual payoff gradient $\payfield_{\play}(\denmat_{\play,\run})$ \needref. 
%However, in an online learning framework, it is more realistic to consider that players observe only the impact of the \emph{realized} outcome of their actions.
%This feedback model is widely used in online optimization and game-theoretic learning \needref and is known as \emph{bandit} feedback \cite{SS11}.
%In this work, we drop the full payoff observation assumption and assume that each player $\play \in \players$ receives as feedback only the realized value of their observable, $\payobs_{\play}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In contrast to finite games with bandit feedback, where the standard approach for players to reconstruct their payoff vectors is through the \acdef{IWE} \needref, we assume that players employ a \acdef{SPSA} method introduced by \cite{Spa92}, which is described in detail next. 
%The reason for this stark difference between the classical and the quantum regime is that in the latter there is a \emph{continuum} of pure states available to every player, while in the former there is only a \emph{finite} set of pure actions. 

\subsection{The SPSA Method in Quantum Games}
To illustrate the intuition of the \ac{SPSA} method, first, consider a 1-dimensional differentiable function $f:\R \to \R$ and a point $x \in \R$. Then, for error tolerance $\radius > 0$, a single-point estimate of the derivative of $f$ at $x$ is given by the expression
\begin{equation}
\hat f_x= \frac{1}{\radius}f(x+\radius s) s
\end{equation}
where $s$ is drawn from $\{\pm1\}$ uniformly at random. Then, $\hat f_x$ is an estimator of the ``discrete derivative''
\begin{equation}
\label{eq:1-point-der}
\ex[\hat f_x] = \frac{f(x+\radius) - f(x-\radius)}{2\radius} 
\end{equation}
Note, that the above estimator requires the evaluation of $f$ at a single point only, \ie $f(x+\radius)$ or $f(x+\radius)$. Going to higher dimensions, letting $f: \R^d \to \R$ be a Lipschitz continuous, $\{e_1,\dots,e_d \}$ be the standard basis of $\R^d$ and $s$ drawn from $\{\pm e_1,\dots,\pm e_d \}$ uniformly at random, the estimator
\begin{equation}
\label{eq:1-point-dif}
\hat f_x = \frac{d}{\radius}f(x+\radius s) s
\end{equation}
is a $\bigoh(\radius)$-approximation of the gradient, \ie $\dnorm{\ex[\hat f_x] - \nabla f(x)} = \bigoh(\radius)$.

%\begin{remark}
%For the rest of the section, we focus on player $\play$ and drop the indices altogether, for notational convenience.
%\end{remark}
%\vspace{-0.5em}
In order to utilize an \ac{SPSA} estimator for a function over the set of density matrices $\denmats$ in $\herm[\vdim]$, we need to ensure two things: \textit{(i)} the feasibility of the \emph{sampling direction}, and \textit{(ii)} the feasibility of the \emph{evaluation point}. The first caveat is due to the fact that the set of the density matrices forms a lower dimensional manifold in the set of Hermitian operators, and therefore, not all directions from a base of $\herm[\vdim]$ are feasible. The second one is due to the fact that $\denmats$ is bounded, thus, even if the sampling direction is feasible, the evaluation point can lie outside the set $\denmats$. 
\vspace{-0.5em}

\para{Sampling Directions}
To account for the first restriction, we will construct an orthonormal basis of the affine hull of $\denmats_{0}$, where $\denmats_{0}= \setdef{\denmat \in\psd[\vdim]}{\tr\denmat = 0}$, and $\aff(\denmats_0)$ is the subspace of $\herm[\vdim]$ with all elements having trace equal to $0$, \ie $\aff(\denmats_{0}) = \setdef{\denmat \in\herm[\vdim]}{\tr\denmat = 0}$.
%\begin{equation}
%\label{eq:denmats-0}
%\denmats_{0}
%	= \setdef{\denmat \in\psd[\vdim]}{\tr\denmat = 0}
%\end{equation}
%and, $\aff(\denmats_0)$ is the subspace of $\herm[\vdim]$ with all elements having trace equal to $0$, \ie
%\begin{equation}
%\label{eq:aff-denmats-0}
%\aff(\denmats_{0})
%	= \setdef{\denmat \in\herm[\vdim]}{\tr\denmat = 0}
%\end{equation}
Note that if $\diagbasis \in \aff(\denmats_0)$ then for any $\denmat \in \herm[\vdim]$ it holds
\begin {enumerate*} [label=(\itshape\alph*\upshape)]
\item
$\denmat + \diagbasis \in \herm[\vdim]$, and
\item
$\trof{\denmat + \diagbasis} = \trof{\denmat}$.
\end {enumerate*} 

Denoting by $\diracmat_{k\ell} \in \herm[\vdim]$ the matrix with $1$ in the $(k,\ell)$-position and $0$'s everywhere else, it is easy to see that the set $\big\{\{\diracmat_{jj}\}_{j=1}^{\vdim} \{\nondiagbasis_{k\ell}\}_{k<\ell}, \{\tilde\nondiagbasis_{k\ell}\}_{k<\ell}\big\}$ is an orthonormal basis of $\herm[\vdim]$, where
\begin{align}
%\diagbasis_j & = \diracmat_{jj} \\
\nondiagbasis_{k\ell} = \frac{1}{\sqrt{2}}\diracmat_{k\ell} +  \frac{1}{\sqrt{2}}\diracmat_{k\ell} \quad & \text{and} \quad
\tilde\nondiagbasis_{k\ell} = \frac{i}{\sqrt{2}}\diracmat_{k\ell} - \frac{i}{\sqrt{2}}\diracmat_{k\ell}
\end{align}
for $1\leq k < \ell\leq\vdim$, where $i$ is the imaginary unit with $i^2 = -1$. The next proposition provides a basis for the subspace $\aff(\denmats_0)$, whose proof lies in the appendix \cref{sec:appendix}.

\begin{restatable}{proposition}{basis}
\label{prop:basis}
Let $\diagbasis_j$ be defined as $\,\diagbasis_j = \frac{1}{\sqrt{j(j+1)}}\parens*{\diagbasis_1 + \dots + \diagbasis_j - j\diagbasis_{j+1}}\,$
%\begin{equation}
%\diagbasis_j = \frac{1}{\sqrt{j(j+1)}}\parens*{\diagbasis_1 + \dots + \diagbasis_j - j\diagbasis_{j+1}}
%\end{equation}
for $j = 1,\dots,\vdim-1$. 
Then, the set $\bvecs = \braces*{\{\diagbasis_j\}_{j=1}^{\vdim-1}, \{\nondiagbasis_{k\ell}\}_{k<\ell}, \{\tilde\nondiagbasis_{k\ell}\}_{k<\ell}}$ is an orthonormal basis of $\aff(\denmats_0)$.% and $\dim(\aff(\denmats_0)) = \vdim^2 - 1$.
\end{restatable}

\para{Feasibility Adjustment}
After establishing an orthonormal basis for $\aff(\denmats_0)$ as per \cref{prop:basis}, and following the idea as in \eqref{eq:1-point-dif}, we readily get that for any $\denmat \in \denmats$, any $\dir \in \dirs \defeq \big\{\{\pm\diagbasis_j\}_{j=1}^{\vdim-1}, \{\pm\nondiagbasis_{k\ell}\}_{k<\ell}, \{\pm\tilde\nondiagbasis_{k\ell}\}_{k<\ell}\big\}$ and $\radius > 0$, the matrix $\denmat + \radius\dir$ belongs to $\aff(\denmats)$.
However, depending on the value of $\radius$ and the distance of $\denmat$ from the boundary of $\denmats$, the point $\denmat + \radius\dir \in \herm[\vdim]$ may fail to lie in $\denmats$ due to violation of the positive-semidefinite condition. Hence, we now treat the latter restriction, \ie the feasibility of the \emph{evaluation point}. 

The idea is to transfer the point $\denmat$ towards the interior of $\denmats$ and move along the sampled direction from there. For this, we need to find a reference point $\refmat \in \relint(\denmats)$ and a safety net $\safe >0$ such that $\refmat + \safe\dir \in \denmats$ for any $\dir \in \dirs$. Then, for $\radius \in (0,r)$, the point  
\begin{equation}
\label{eq:pivot}
\pivot \defeq \denmat + \frac{\radius}{\safe}(\refmat - \denmat)
\end{equation}
lies in $\relint(\denmats)$, and moving along $\dir \in \dirs$, we readily get a point in $\denmats$, since:
\begin{align}
\label{eq:perturbation}
\pivot + \radius\dir & = (1-\frac{\radius}{\safe})\denmat + \frac{\radius}{\safe}(\refmat + \safe\dir) \in \denmats
\end{align}
as a convex combination of two elements in $\denmats$. The following proposition provides an exact expression for $\refmat$ and $\safe$, whose proof lies in the appendix \cref{sec:appendix}.

\begin{restatable}{proposition}{adjustment}
\label{prop:adjustment}
Let $\refmat \in \denmats$ be defined as $\refmat= \frac{1}{{\vdim}}\sum_{j = 1}^{\vdim}\diracmat_{jj}$.
%\begin{equation}
%\refmat= \frac{1}{{\vdim}}\sum_{j = 1}^{\vdim}\diracmat_{jj}
%\end{equation}
Then, for $\safe = \min\braces*{\frac{1}{\sqrt{\vdim(\vdim-1)}}, \frac{\sqrt{2}}{\vdim}}
$, it holds that $\refmat + \safe\dir \in \denmats$ for any direction $\dir \in \dirs$.
\end{restatable}
To illustrate how our method can be deployed, we begin with the simpler payoff-based case, where each player may observe $\pay_{\play}(\denmat)$, and we defer the full problem to the next section.


\subsection{Payoff-based Learning in Quantum Games}

The previous procedure applies to each player $\play \in \players$, and using \cref{prop:adjustment}, we obtain a reference point, $\refmat_\play$, and a safety net, $\safe_\play$, per player.
At this point we are ready to provide the sequence of events for constructing the approximate payoff gradients.
Given state $\denmat_\run$ and sampling radius $\radius_\run$, the steps for generating $\payfield_{\play,\run}$ for every player $\play \in \players$, proceed as follows:
\begin{enumerate}[\textbf{Step} 1]
\item
Each player $\play \in \players$ draws a sampling direction $\dir_{\play,\run}$ from $\bvecs_{\play}^{\pm}$ uniformly at random.
\item
Instead of moving towards $\dir_{\play,\run}$ form $\denmat_{\play,\run}$, \ie playing $\denmat_{\play,\run} + \radius_\run\dir_{\play,\run}$, perform the feasibility adjustment as per \eqref{eq:pivot},
and play $\hat\denmat_{\play,\run} \defeq (1-{\radius_\run}/{\safe_\play})\denmat_{\play,\run} + {\radius_\run}/{\safe_\play}\cdot(\refmat_\play + \safe_\play\dir_{\play,\run})$ to ensure the feasibility of the evaluation point.
\item
Under $\hat\denmat_\run$, each $\outcome \in \outcomes$ is occurred with probability $\pdist_{\outcome}(\hat\denmat_\run)$. 
Player $\play \in \players$ observes $\payobs_{\play}(\outcome_\run)$, where $\outcome_\run$ is the random outcome.
\item
Approximate $\payfield_{\play}(\denmat_\run)$  using the estimator:
\begin{equation}
\label{eq:Q-SPSA}
\tag{Q-SPSA}
\paysignal_{\play,\run} \defeq\frac{(\vdim_{\play}^2-1)}{\radius_\run} \payobs_{\play}(\outcome_\run)\dir_{\play,\run}
\end{equation}
\end{enumerate}
Finally, putting all the pieces together, we provide the pseudocode implementation of the \ac{MMW} with bandit feedback for quantum games in \cref{alg:Q-SPSA}.
\begin{algorithm}[H]
\caption{MMW with bandit feedback}
\label{alg:Q-SPSA}
\begin{algorithmic}[1]
	\State
	Initialize: safety net $\safe_\play$ and reference point $\refmat_{\play}$ for $\play \in \players$ , step-size $\step_\run$, sampling radius $\radius_\run$, initial point $\init$
	\For{$\run = 1,2,\dots$ simultaneously for all players $\play \in \players$}
		\State
		sample $\dir_{\play,\run}$ uniformly from $\bvecs_{\play}^{\pm}$	
		\State
		play $\hat\denmat_{\play,\run} \defeq (1-{\radius_\run}/{\safe_\play})\denmat_{\play,\run} + {\radius_\run}/{\safe_\play}\cdot(\refmat_\play + \safe_\play\dir_{\play,\run})$		
		\State
		receive $\hat\pay_{\play,\run} \defeq \payobs_{\play}(\outcome_\run)$
		\State
		set $\paysignal_{\play,\run} \defeq {(\vdim_{\play}^2-1)}/{\radius_\run} \cdot \hat\pay_{\play,\run}\dir_{\play,\run}$
		\State
		update $\denmat_{\play,\run+1} \leftarrow \denmat_{\play,\run}\exp(\step_\run\paysignal_{\play,\run})/\trof*{ \denmat_{\play,\run}\exp(\step_\run\paysignal_{\play,\run})}$
	\EndFor
\end{algorithmic}
\end{algorithm}
Letting $\filter_\run = \sigma(\init,\dots,\curr)$ be the natural filtration generated by the sequence of play, the \eqref{eq:Q-SPSA} estimator enjoys the following statistical bounds.
%For the analysis of \cref{alg:Q-SPSA} we need the following statistical bounds of the \eqref{eq:Q-SPSA} estimator.
\begin{restatable}{proposition}{statistics}
\label{prop:Q-SPSA-statistics}
The estimator \eqref{eq:Q-SPSA} satisfies the following statistical properties:
\begin{equation}
\label{eq:Q-SPSA-statistics}
\text{(i)}\quad
\dnorm*{\ex\bracks*{\paysignal_{\play,\run} \mid \filter_\run} - \payfield_\play(\denmat_\run)} = \bigoh(\radius_\run)
\quad \text{and} \quad \text{(ii)}\quad
\ex\bracks*{\dnorm*{\paysignal_{\play,\run}}^2  \mid \filter_\run} = \bigoh(1/\radius_{\run}^{2})
\end{equation}
%\begin{equation}
%\label{eq:variance}
%\ex\bracks*{\dnorm*{\paysignal_{\play,\run}}^2  \mid \filter_\run} = \bigoh(1/\radius_{\run}^{2})
%\end{equation}
\end{restatable}

At this point, we are ready to proceed to our main results. 
\para{Zero-sum Quantum Games}
After establishing the statistical properties of \eqref{eq:Q-SPSA}, we are ready to present our theorem on the convergence of the \emph{ergodic-averaged} sequence
\begin{equation}
\label{eq:ergodic}
\ergodic_\run = \parens*{\frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{1,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}, \frac{\sum_{\runalt = 1}^\run \step_\runalt \denmat_{2,\runalt}}{\sum_{\runalt = 1}^\run \step_\runalt}}
\end{equation}
of the \ac{MMW} with bandit feedback for a zero-sum quantum game. 
\begin{restatable}{theorem}{banditzero}
\label{eq:bandit-zero}
Consider a 2-player zero-sum quantum game, where each player follows \eqref{eq:MMW} with bandit feedback, as per \cref{alg:Q-SPSA}, with learning-rate and sampling radius parameters satisfying
\begin{equation}
\label{eq:hyperparameters-zero}
\text{(i)}\quad
\sum_{\run = 1}^\infty \step_\run = \infty,
\quad \text{(ii)}\quad
\sum_{\run = 1}^\infty \step_\run \radius_\run < \infty,
\quad \text{and} \quad \text{(ii)}\quad
\sum_{\run = 1}^\infty \step_{\run}^2/\radius_{\run}^2 < \infty
\end{equation}
Then, the ergodic sequence of play \eqref{eq:ergodic} converges to a \ac{NE} point with probability 1. 
Specifically,
for $\step_\run \propto \run^{-\pexp}$ and $\radius_\run \propto \run^{-\qexp}$ such that $\pexp \in (3/4,1)$ and $\qexp \in (1-\pexp, \pexp - 1/2)$, the rate of convergence is $\bigoh(\run^{1-\pexp})$.
%\begin{enumerate}
%\item
%For $\step_\run \propto \run^{-\pexp}$ and $\radius_\run \propto \run^{-\qexp}$ such that $\pexp \in (3/4,1)$ and $\qexp \in (1-\pexp, \pexp - 1/2)$, the rate of convergence is $\bigoh(\run^{1-\pexp})$.
%\item
%\end{enumerate}
%satisfying (i) $\sum_{\run = 1}^\infty \step_\run = \infty$, and (ii) $\sum_{\run = 1}^\infty \step_{\run}^2 < \infty$.
%\begin{equation}
%\sum_{\run = 1}^\infty \step_\run = \infty
%\quad \text{and} \quad
%\sum_{\run = 1}^\infty \step_{\run}^2 = \infty
%\end{equation}
\end{restatable}

\para{General Quantum Games}
A key characteristic to keep in mind is that a quantum game may admit several Nash equilibria, thus, it is not reasonable to expect a global convergence result that applies
to all games.
In light of this, we focus on quantum states that satisfy the property of variational stability - an equilibrium refinement in the spirit of the seminal concept of \emph{evolutionary stability} \cite{MP73,May82} - as formalized below.
\begin{definition}
\label{def:VS}
We say that $\eq\in\denmats$ is \emph{\textpar{locally} variationally stable} if there exists a neighborhood $\pnhd$ of $\eq$ in $\denmats$ such that
\begin{equation}
\label{eq:VS}
\tag{VS}
\trof{\payfield(\denmat) (\denmat - \eq)}
	< 0
	\quad
	\text{for all $\denmat\in\pnhd\exclude{\eq}$}.
\end{equation}
\end{definition}

The \eqref{eq:VS} condition allows us to consider \emph{last-iterate} convergence results in general quantum games, due to a consistent drift on the sequence of play towards the variationally stable point $\eq$ within a neighborhood of the latter. Formally, we have the following result.

\begin{restatable}{theorem}{banditgeneral}
Consider a $\nPlayers$-player quantum game and let $\eq$ be a variational stable point, as per \eqref{eq:VS}. Fix some confidence level $\conf \in (0,1)$. 
If each player follows \eqref{eq:MMW} with bandit feedback, as per \cref{alg:Q-SPSA}, with learning-rate and sampling radius parameters satisfying
\begin{equation}
\label{eq:hyperparameters-general}
\text{(i)}\quad
\sum_{\run = 1}^\infty \step_\run = \infty,
\quad \text{(ii)}\quad
\sum_{\run = 1}^\infty \step_\run \radius_\run < \infty,
\quad \text{and} \quad \text{(ii)}\quad
\sum_{\run = 1}^\infty \step_{\run}^2/\radius_{\run}^2 < \infty
\end{equation}
then, there exists a neighborhood $\nhd$ of $\eq$ in $\denmats$ such that
\begin{equation}
\probof*{\curr \to \eq \given \init \in \nhd} \geq 1-\conf
\end{equation} 
\end{restatable}
%\begin {enumerate*} [label=(\itshape i\upshape)] 
%\item 
%$\diagbasis_i = \diracmat_{ii}$,
%\item
%$\nondiagbasis_{ij} = \frac{1}{\sqrt{2}}\diracmat_{ij} +  \frac{1}{\sqrt{2}}\diracmat_{ji}$, and
%\item 
%$\tilde\nondiagbasis_{ij} = \frac{i}{\sqrt{2}}\diracmat_{ij} - \frac{i}{\sqrt{2}}\diracmat_{ji}$
%\end{enumerate*}
%Note, that the above estimate requires the evaluation of $f$ at two points, $f(x+\radius)$ and $f(x+\radius)$. To further reduce to single-point approximation, one can randomize the point of evaluation between $x\pm\radius$. More rigorously, letting $s $ be ${\pm 1}$ uniformly at random, the quantity is an unbiased estimator of \eqref{eq:2-point-der}. 

==> Body/Prelims-Nplayers.tex <==
%----------------------------------------------------------------------
%%% PRELIMS
%----------------------------------------------------------------------
% !TEX root = ../Main.tex

%We start by briefly reviewing some basics of quantum game theory and introducing the necessary context for our results.
To begin, we will provide a brief overview of the fundamentals of quantum game theory and establish the required background context for our results.
%----------------------------------------------------------------------
%% Notation
%----------------------------------------------------------------------
\para{Notation}
Given a (complex) Hilbert space $\hilbert$, we will use Dirac's bra-ket notation to denote an element $\ket{\quant}$ of $\hilbert$ and its adjoint $\bra{\quant}$;
otherwise, when a basis is implied by the context, we will use the dagger notation ``$\dag$'' to denote the Hermitian transpose $\quant^{\dag}$ of $\quant$.
We will also write $\herm[\vdim]$ for the space of $\vdim\times\vdim$ Hermitian matrices, and $\psd[\vdim]$ for the cone of positive-semidefinite matrices in $\herm[\vdim]$.
%Finally, given a real function $\fun\from\R\to\R$ and a Hermitian matrix $\denmat\in\herm[\vdim]$ with unitary eigen-decomposition $\denmat = \sum_{\coord=1}^{\vdim} \denval_{\coord} \denvec_{\coord} \denvec_{\coord}^{\dag}$,
%we will write $\fun(\denmat)$ for the matrix $\fun(\denmat) = \sum_{\coord=1}^{\vdim} \fun(\denval_{\coord}) \denvec_{\coord}\denvec_{\coord}^{\dag}$.


%----------------------------------------------------------------------
%% Quantum games
%----------------------------------------------------------------------
\para{Quantum games}

Following \cite{EWL99,GW07}, a \emph{quantum game} consists of the following primitives:
\begin{enumerate}
\item
A finite set of \emph{players} $\play\in\players = \{1,\dotsc,\nPlayers\}$.
\item
Each player $\play\in\players$ has access to a complex Hilbert space $\hilbert_{\play} \cong \C^{\vdim_{\play}}$ describing the set of (pure) \emph{quantum states} available to the player (typically a discrete register of qubits).
A quantum state is an element $\quant_{\play}$ of $\hilbert_{\play}$ with unit norm, so the set of pure states is the unit sphere $\quants_{\play} \defeq \setdef{\quant_{\play}\in\hilbert_{\play}}{\norm{\quant_{\play}}=1}$ of $\hilbert_{\play}$.
We will write $\quants \defeq \prod_{\play} \quants_{\play}$ for the space of all ensembles $\quant = (\quant_{1},\dotsc,\quant_{\nPlayers})$ of pure states $\quant_{\play}\in\quants_{\play}$ that are independently prepared by each $\play\in\players$.
\item
The rewards that players receive are based on their individual \emph{payoff functions} $\pay_{\play}\from\quants \to \R$, which are derived through a \acdef{POVM} quantum measurement process, that unfolds as follows \cite{CN10}.
%These payoff functions are not arbitrary, but are obtained from a joint \acdef{POVM} quantum measurement process that unfolds as follows \cite{CN10}:
Given a \emph{finite} set of \emph{measurement outcomes} $\outcomes$ that a referee can observe from the players' quantum states (\eg measure a player-prepared qubit to be ``up'' or ``down''), each outcome $\outcome\in\outcomes$ is associated to a positive semi-definite operator $\povm_{\outcome}\from\hilbert\to\hilbert$ defined on the tensor product $\hilbert \defeq \bigotimes_{\play} \hilbert_{\play}$ of the players' individual state spaces;
%The family $\povm = (\povm_{\outcome})_{\outcome\in\outcomes}$ is referred to as a \acdef{POVM}.
we further assume that $\sum_{\outcome\in\outcomes} \povm_{\outcome} = \eye$, thus, the probability of observing $\outcome\in\outcomes$ at state $\quant\in\quants$ is
\begin{equation}
\pdist_{\outcome}(\quant)
	= \bra{\quant_{1}\otimes\dotsm\otimes\quant_{\nPlayers}}
		\povm_{\outcome}
		\ket{\quant_{1}\otimes\dotsm\otimes\quant_{\nPlayers}}
\end{equation}
%Given such a \acdef{POVM} $\povm = (\povm_{\outcome})_{\outcome\in\outcomes}$ on $\hilbert$,
Each player's payoff is generated by this measurement process via a \emph{payoff observable} $\payobs_{\play}\from\outcomes\to\R$;
%known as a \emph{payoff observable};
in this context, $\pay_{\play}(\quant)$ denotes the player's expected payoff at state $\quant\in\quants$, namely
\begin{equation}
\label{eq:pay-pure}
\pay_{\play}(\quant)
	\defeq \obs{\payobs_{\play}}
	\equiv \insum_{\outcome} \pdist_{\outcome}(\quant) \, \payobs_{\play}(\outcome).
\end{equation}
\end{enumerate}
A \emph{quantum game}
%\textendash\ also known as a quantum \emph{refereed} game in reference to the underlying measurement process \textendash\
is then defined as a tuple $\qgame \equiv \qgamefull$ with players, quantum states, and payoff functions as above.


%----------------------------------------------------------------------
%% Mixing
%----------------------------------------------------------------------
\para{Mixed states}
Apart from pure states, each player $\play\in\players$ has the ability to prepare probabilistic mixtures, also known as \emph{mixed states}. 
These mixed states differ from mixed strategies used in classical, finite games as they do not correspond to convex combinations of their pure counterparts;
%In addition to pure states, each player $\play\in\players$ can also prepare probabilistic mixtures thereof, known as \emph{mixed states}.
%In contrast to mixed strategies in classical, finite games, these mixed states are \emph{not} convex combinations of their pure counterparts;
in contrast, given a family of pure quantum states $\quant_{\play\pure_{\play}} \in \quants_{\play}$ indexed by $\pure_{\play}\in\pures_{\play}$, a mixed state is described by a \emph{density matrix} of the form
\begin{equation}
\label{eq:denmat}
\denmat_{\play}
	= \smashoperator{\sum_{\pure_{\play}\in\pures_{\play}}}
		\strat_{\play\pure_{\play}}
		\ket{\quant_{\play\pure_{\play}}}
		\bra{\quant_{\play\pure_{\play}}}
\end{equation}
where
%$\pures_{\play}$ is a family of indices,
%$\quant_{\play\pure_{\play}} \in \quants_{\play}$ are the states being mixed,
$\strat_{\play\pure_{\play}} \geq 0$ is the mixing weight of $\quant_{\play\pure_{\play}}$,
and
such that $\tr\denmat_{\play} = 1$. % (the states $\quant_{\play\pure_{\play}}$ are not assumed to be orthogonal in this context).
By Born's rule, this means that if each player $\play\in\players$ prepares a density matrix $\denmat_{\play}$ as per \eqref{eq:denmat}, the probability of the outcome $\outcome\in\outcomes$ under $\denmat = (\denmat_{1},\dotsc,\denmat_{\nPlayers})$ will be
\begin{equation}
\label{eq:prob-density}
\pdist_{\outcome}(\denmat)
	= \sum_{\pure} \strat_{\pure} \bra{\quant_{\pure}} \povm_{\outcome} \ket{\quant_{\pure}},
%	= \sum_{\pure_{1}\in\pures_{1}} \dotsi \sum_{\pure_{\nPlayers}\in\pures_{\nPlayers}}
%		\strat_{\pure_{1}} \dotsm \strat_{\pure_{\nPlayers}}
\end{equation}
where, in multi-index notation,
$\pure = (\pure_{1},\dotsc,\pure_{\nPlayers})$,
$\strat_{\pure} = \prod_{\play} \strat_{\play\pure_{\play}}$,
and
%$\quant_{\pure} = \quant_{1,\pure_{1}} \otimes \dotsm \otimes \quant_{\nPlayers,\pure_{\nPlayers}}$.
$\quant_{\pure} = \bigotimes_{\play} \quant_{\play\pure_{\play}}$.
Therefore, in a slight abuse of notation, the expected payoff of player $\play\in\players$ under $\denmat$ will be
\begin{align}
\label{eq:pay-mix}
\pay_{\play}(\denmat)
	&= \sum_{\outcome\in\outcomes} \sum_{\pure\in\pures}
		\strat_{\pure} \pdist_{\outcome}(\quant_{\pure}) \, \payobs_{\play}(\outcome)
	= \sum_{\pure\in\pures} \strat_{\pure}
		\pay_{\play}(\quant_{\pure})
	%\notag\\
	% &= \smashoperator{\sum_{\pure_{1}\in\pures_{1}}} \:\dotsi\: \smashoperator{\sum_{\pure_{\nPlayers}\in\pures_{\nPlayers}}}
	% 	\strat_{\pure_{1}} \!\dotsm \strat_{\pure_{\nPlayers}}\,
	% 	\pay_{\play}(\quant_{\pure_{1}},\dotsc,\quant_{\pure_{\nPlayers}}).
%	\sum_{\outcome\in\outcomes} 
\end{align}
Equivalently, we can write the above as:
\begin{align}
\label{eq:pay-mat}
\pay_{\play}(\denmat)
    &= \sum_{\outcome\in\outcomes}\payobs_{\play}(\outcome) \trof{\povm_{\outcome} \denmat_{1}\otimes\dotsm\otimes\denmat_{\nPlayers}}
    \notag\\
    &= \trof{\paymat_{\play} \denmat_{1}\otimes\dotsm\otimes\denmat_{\nPlayers}}
\end{align}
where the tensor $\paymat_i = \sum_{\outcome\in\outcomes}\payobs_{\play}(\outcome)\povm_{\outcome} \in \hilbert$ for $\play \in \players$ incorporates all the payoff information of the game and is the quantum equivalent of the ``payoff matrix'' of player $\play\in\players$.
In light of this, \eqref{eq:pay-mat} gives a clearer and more succint representation of the payoff structure of $\qgame$ - see also \eqref{eq:pay-lin} below.


%----------------------------------------------------------------------
%% Quantum vs. finite
%----------------------------------------------------------------------
\para{Contrasting to other classes of games}

The expression \eqref{eq:pay-mix} for a player's expected payoff under a mixed state appears similar to mixed extensions of classical finite games. %, but this association is very tenuous.
Nevertheless, the resemblance is tenuous, and the key conceptual dissimilarities are as follows:
%From a conceptual standpoint, the principal differences are as follows:
\begin{enumerate}[leftmargin=0.5cm]
%[\upshape(\itshape\alph*\upshape)]
\item
There is an infinite continuum of pure states $\quant\in\quants$, unlike a finite number thereof in finite games.
\item
The decomposition \eqref{eq:denmat} of a density matrix into pure states is not exclusive; 
there can be different sets of pure states and corresponding mixing weights that produce the same density matrix.
%The decomposition \eqref{eq:denmat} of a density matrix into pure states is not unique;
%generically, there may be a continuum of (non-equivalent) families of pure states and mixing weights giving rise to the same density matrix.
%(this is a consequence of the well-known Schrödinger\textendash HJW theorem).
\item
The convex superposition $\coef\quant + (1-\coef)\quantalt$ of two pure states $\quant$ and $\quantalt$ may give rise to quantum interference terms of the form $\ket{\quant}\bra{\quantalt}$ and $\ket{\quantalt}\bra{\quant}$ in the induced payoff with no analogue in finite games.
\end{enumerate}

\para{Continuous game reformulation}
As a result of the earlier discussion, considering a quantum game as a ``tensorial'' extension of a finite game can be misleading.
For our objectives, it would be more accurate to treat a quantum game as a \emph{continuous game} where each player $\play\in\players$ controls a matrix variable $\denmat_{\play}$ drawn from the ``spectraplex''
%Instead, it would be clearer for our purposes to view a quantum game as a \emph{continuous game} where each player $\play\in\players$ controls a matrix variable $\denmat_{\play}$ drawn from the ``spectraplex''
\begin{equation}
\label{eq:denmats}
\denmats_{\play}
	= \setdef{\denmat_{\play}\in\psd[\vdim_{\play}]}{\tr\denmat_{\play} = 1}
\end{equation}
and the player's payoff function $\pay_{\play}\from\denmats \equiv \prod_{\playalt} \denmats_{\playalt} \to \R$ is linear in every player's density matrix $\denmat_{\playalt} \in \denmats_{\playalt}$, $\playalt\in\players$.  
Since $\pay_{\play}$ is linear in $\denmat_{\play}$, letting
\begin{align}
\label{eq:payfield-def}
    \payfield_{\play}(\denmat)
	& \defeq \nabla_{\denmat_{\play}^{\top}} \pay_{\play}(\denmat) 
	= \trof{\paymat_{\play} \denmat_{1}\otimes\denmat_{\play-1} \otimes \eye \otimes \denmat_{\play+1} \otimes \dotsm \otimes\denmat_{\nPlayers}}
\end{align}
denote the individual payoff gradient of player $\play$,
% (where the trace is taken over all $\playalt\neq\play$),
%the $\play$-th block $\payfield_{\play}(\denmat)$ of $\payfield(\denmat)$ does not depend on $\denmat_{\play}$, thus:
we can write the payoff of player $\play$ in terms of the gradient $\payfield_\play$ as:
\begin{equation}
\label{eq:pay-lin}
\pay_{\play}(\denmat_{\play};\denmat_{-\play})
	= \trof{\denmat_{\play} \payfield_{\play}(\denmat)}
	\quad
	\text{for all $\denmat\in\denmats$}.
\end{equation}
In view of the above, we are now ready to proceed to the concept of Nash equilibrium.
%(or, equivalently, linear in $\denmat_{1}\otimes\dotsm\otimes\denmat_{\nPlayers}$).


%----------------------------------------------------------------------
%% Equilibrium
%----------------------------------------------------------------------
\para{\Acl{NE}}

In our quantum setting, the standard concept of a \acdef{NE} characterizes mixed quantum states $\eq \in \denmats$, which no player has incentive to unilaterally deviate from, in the sense that
\begin{equation}
\label{eq:Nash}
\tag{NE}
\pay_{\play}(\eq)
	\geq \pay_{\play}(\denmat_{\play};\eq_{-\play})
	\quad
	\text{for all $\denmat_{\play}\in\denmats_{\play}$, $\play\in\players$}
\end{equation}
where we write $(\denmat_{\play};\denmat_{-\play}) = (\denmat_{1},\dots,\denmat_{\play},\dotsc,\denmat_{\nPlayers})$ for the choice of player $\play$ relative to all other players.
Since $\denmats_{\play}$ is convex and $\pay_{\play}$ is linear in $\denmat_{\play}$, the existence of \aclp{NE} is derived from the seminal theorem of \citet{Deb52}. 
Standard arguments \cite{FP03,SFPP10} show that the \aclp{NE} of $\qgame$ are precisely the solutions of the \acl{VI}
\begin{equation}
\label{eq:VI}
\tag{VI}
\trof{\payfield(\eq) (\denmat - \eq)}
	\leq 0
	\quad
	\text{for all $\denmat\in\denmats$}
\end{equation}
where $\payfield(\denmat) = (\payfield_{1}(\denmat),\dotsc,\payfield_{\nPlayers}(\denmat))$.
We will use this equivalence freely in the sequel.



